Achieving Pareto Optimality using Efficient Parameter Reduction for DNNs in Resource-Constrained Edge Environment

This paper proposes an optimization of an existing Deep Neural Network (DNN) that improves its hardware utilization and facilitates on-device training for resource-constrained edge environments. We implement efficient parameter reduction strategies on Xception that shrink the model size without sacrificing accuracy, thus decreasing memory utilization during training. We evaluate our model in two experiments: Caltech-101 image classification and PCB defect detection and compare its performance against the original Xception and lightweight models, EfficientNetV2B1 and MobileNetV2. The results of the Caltech-101 image classification show that our model has a better test accuracy (76.21%) than Xception (75.89%), uses less memory on average (847.9MB) than Xception (874.6MB), and has faster training and inference times. The lightweight models overfit with EfficientNetV2B1 having a 30.52% test accuracy and MobileNetV2 having a 58.11% test accuracy. Both lightweight models have better memory usage than our model and Xception. On the PCB defect detection, our model has the best test accuracy (90.30%), compared to Xception (88.10%), EfficientNetV2B1 (55.25%), and MobileNetV2 (50.50%). MobileNetV2 has the least average memory usage (849.4MB), followed by our model (865.8MB), then EfficientNetV2B1 (874.8MB), and Xception has the highest (893.6MB). We further experiment with pre-trained weights and observe that memory usage decreases thereby showing the benefits of transfer learning. A Pareto analysis of the models' performance shows that our optimized model architecture satisfies accuracy and low memory utilization objectives.

==> Contents/tables/edge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccllll@{}}
\toprule
\multicolumn{2}{c}{} &
  \multicolumn{1}{c}{Embedded Edge   Devices} &
  \multicolumn{1}{c}{Edge Nodes/   Edge Servers/ Edge Computers/ Micro Data} &
  \multicolumn{1}{c}{Edge Routers/   Edge Switches/ Edge Gateways} &
  \multicolumn{1}{c}{Edge Accelerator} \\ \midrule
\multicolumn{1}{|c|}{\multirow{2}{*}{Processing Power}} &
  \multicolumn{1}{c|}{CPU} &
  \multicolumn{1}{l|}{Low-power   processors} &
  \multicolumn{1}{l|}{General-purpose   processors} &
  \multicolumn{1}{l|}{Customized   processors} &
  \multicolumn{1}{l|}{Specialized   AI processors} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{GPU} &
  \multicolumn{1}{l|}{Not   applicable} &
  \multicolumn{1}{l|}{Not   applicable} &
  \multicolumn{1}{l|}{Not   applicable} &
  \multicolumn{1}{l|}{Optimized   GPU architecture} \\ \midrule
\multicolumn{2}{|c|}{Memory} &
  \multicolumn{1}{l|}{Limited   RAM} &
  \multicolumn{1}{l|}{Moderate   to high RAM} &
  \multicolumn{1}{l|}{Moderate   to high RAM} &
  \multicolumn{1}{l|}{Moderate   to high RAM} \\ \midrule
\multicolumn{2}{|c|}{Storage} &
  \multicolumn{1}{l|}{Limited   flash storage} &
  \multicolumn{1}{l|}{Moderate   to high storage (HDD/SSD)} &
  \multicolumn{1}{l|}{Moderate   to high storage (HDD/SSD)} &
  \multicolumn{1}{l|}{Limited   storage (on-chip)} \\ \midrule
\multicolumn{2}{|c|}{Network} &
  \multicolumn{1}{l|}{Basic   connectivity} &
  \multicolumn{1}{l|}{Ethernet,   Wi-Fi, Cellular} &
  \multicolumn{1}{l|}{Ethernet,   Wi-Fi, Cellular} &
  \multicolumn{1}{l|}{Ethernet,   PCIe} \\ \midrule
\multicolumn{2}{|c|}{AI Support} &
  \multicolumn{1}{l|}{Limited   or no support} &
  \multicolumn{1}{l|}{Can   support AI frameworks and algorithms} &
  \multicolumn{1}{l|}{Limited   support for AI inference} &
  \multicolumn{1}{l|}{Optimized   for AI inference} \\ \midrule
\multicolumn{2}{|c|}{Power/Energy Consumption} &
  \multicolumn{1}{l|}{Low   power consumption} &
  \multicolumn{1}{l|}{Moderate   power consumption} &
  \multicolumn{1}{l|}{Moderate   power consumption} &
  \multicolumn{1}{l|}{Moderate   to high power consumption} \\ \midrule
\multicolumn{1}{|c|}{\multirow{3}{*}{Durability (Environment Resistant)}} &
  \multicolumn{1}{c|}{Shock   vs Vibration} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Temperature} &
  \multicolumn{1}{l|}{No} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{No} \\ \cmidrule(l){2-6} 
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Waterproof} &
  \multicolumn{1}{l|}{No} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{Moderate} &
  \multicolumn{1}{l|}{No} \\ \midrule
\multicolumn{2}{|c|}{Price} &
  \multicolumn{1}{l|}{Low} &
  \multicolumn{1}{l|}{Moderate   to high} &
  \multicolumn{1}{l|}{Moderate   to high} &
  \multicolumn{1}{l|}{High} \\ \midrule
\multicolumn{2}{|c|}{Typical Application} &
  \multicolumn{1}{l|}{Kiosk   machines, Building automation, Environmental monitoring, Industrial robotics} &
  \multicolumn{1}{l|}{Railway   signaling systems, Industrial data centers, Smart cities infrastructure} &
  \multicolumn{1}{l|}{Industrial   control systems, Industrial gateways, Smart manufacturing systems} &
  \multicolumn{1}{l|}{Video   surveillance and analytics, Autonomous vehicles and robotics} \\ \midrule
\multicolumn{2}{|c|}{Areas of Applications} &
  \multicolumn{1}{l|}{Sensor   devices, wearables, IoT devices} &
  \multicolumn{1}{l|}{Edge   computing, cloud offloading, data processing} &
  \multicolumn{1}{l|}{Network   routing, connectivity, data aggregation} &
  \multicolumn{1}{l|}{AI   inference, machine learning} \\ \midrule
\multicolumn{2}{|c|}{Example of Devices} &
  \multicolumn{1}{l|}{Arduino,   Raspberry Pi} &
  \multicolumn{1}{l|}{Industrial   edge servers, NVIDIA Jetson,Dell Edge Gateway} &
  \multicolumn{1}{l|}{Cisco   IoT routers, Juniper Networks} &
  \multicolumn{1}{l|}{NVIDIA   Tesla T4, Google TPU} \\ \midrule
\multicolumn{2}{|c|}{Drawbacks} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{} \\ \midrule
\multicolumn{2}{c}{I/O} &
   &
   &
   &
   \\ \bottomrule
\end{tabular}%
}
% \end{table}

==> Contents/tables/edgeDevice.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{p{5em}p{5em}p{10em}p{12em}p{10em}p{10em}}
\hline
\hline
\multicolumn{2}{c}{} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Embedded} \\ \textbf{Edge Devices}\end{tabular}} &
%\multicolumn{1}{c|}{Embedded Edge Devices} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Nodes {\slash}} \\ \textbf{Edge Servers {\slash}} \\ \textbf{Edge Computers {\slash}} \\ \textbf{Micro Datacenter}\end{tabular}} &
%\multicolumn{1}{c|}{Edge Nodes {\slash} Edge Servers {\slash} Edge Computers {\slash} Micro Data Center} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Routers {\slash}} \\ \textbf{Edge Switches {\slash}} \\ \textbf{Edge Gateways}\end{tabular}} &
%\multicolumn{1}{c|}{Edge Routers {\slash} Edge Switches {\slash} Edge Gateways} &
\multicolumn{1}{c}{\textbf{Edge Accelerators}} \\ \hline
\multicolumn{2}{c}{Processing Power} &
Micro-controller, Low-power processors {\newline}\textit{e.g., AVR, PIC} &
  General purpose processors (up to 64 cores); GPU Supported 
  {\newline} \textit{e.g., Intel Atom, Intel Celeron, Xeon Processor}  &
  General purpose processors (4 to 56 cores); 
  {\newline} \textit{e.g., 2nd Generation Intel Xeon Scalable} &
  Specialized   AI processors; GPU Supported
  {\newline} \textit{e.g., Intel VPU, Google TPU, FPGA, Apple NPU}  \\ \hline
\multicolumn{2}{c}{Memory} &
  Up to 8MB; {\newline} \textit{e.g., SRAM} &
  Up to 256GB; {\newline} \textit{e.g., DDR4 RDIMM{\slash}LR-DIMM} &
  Up to 64GB; {\newline}\textit{e.g., DRAM} &
  Up to 8GB; {\newline} \textit{e.g., GDDR6, SDRAM, LPDDR4} \\ \hline
\multicolumn{2}{c}{Storage} &
  Up to 16MB {\newline} \textit{e.g., MicroSD}& 
  8GB to 6TB; {\newline} \textit{e.g., NVMe, SSD, MicroSD, eMMC} &
  Up to 2TB; {\newline} \textit{e.g., NVMe, SSD, SATA} &
  Up to 128GB; {\newline} \textit{e.g., eMMC, MicroSD}\\ \hline
\multicolumn{2}{c}{Network} &
  Bluetooth, Wi-Fi &
  Ethernet, Wi-Fi, Cellular &
  Ethernet, Wi-Fi, Cellular &
  Ethernet \\ \hline
\multicolumn{2}{c}{I/O} &
  Limited
  {\newline} \textit{e.g., USB, Ethernet} &
  Vary
  {\newline} \textit{PCIe, OCP, LOM, USB, iDRAC network port, Display ports} &
  Vary
  {\newline} \textit{Display ports, USB, uSIM slots, COM, Digital I/O} &
  Vary
  {\newline} \textit{PCIe, USB, HDMI, uSDHC, GPIO} \\ \hline
\multicolumn{2}{c}{AI Optimization} &
  Not Supported &
  Not Supported &
  Not Supported &
  Optimized for AI inference \\ \hline
\multicolumn{2}{c}{Power Consumption} &
  Low &
  Moderate &
  Moderate &
  Moderate to High \\ \hline
\multicolumn{1}{c}{\multirow{3}{*}{Durability}} &
  {\begin{tabular}[c]{@{}c@{}}{Shock \&} \\ {Vibration}\end{tabular}} &
  % Shock\&Vibration &
  Some Application Supports &
  Some Application Supports &
  Some Application Supports &
  Not Supported \\ \cline{2-6} 
\multicolumn{1}{c}{} &
  Temperature &
  -40C to 85C &
  -40C to 85C &
  -20C to 60C &
  -40C to 85C  \\ \cline{2-6} 
\multicolumn{1}{c}{} &
  Waterproof &
  Some Application Supports &
  Some Application Supports &
  Some Application Supports &
  No \\ \hline
\multicolumn{2}{c}{Price} &
  \$ &
  \$\$\$ &
  \$\$\$ &
  \$\$\$\$\$ \\ \hline
\multicolumn{2}{c}{Example of Devices} &
  Arduino &
  Raspberry Pi, Industrial Edge servers, NVIDIA Jetson&
  Cisco IoT routers, Juniper Networks, Dell Edge Gateway  &
  % NVIDIA Tesla T4, 
  Google Coral, Nvidia Jetson Nano, Intel Neural Compute Stick \\ \hline
\multicolumn{2}{c}{Typical Application} &
  Sensor devices, wearables, IoT devices, smart appliances\cite{9904804}\cite{8951147} &  
  Kiosk machines, Building automation, Environmental monitoring, Industrial robotics, Railway signaling systems, Industrial data centers, Smart cities infrastructure\cite{JIANG2020556} &
  Industrial control systems, Industrial gateways, Smart manufacturing systems &
  Video surveillance and analytics, Autonomous vehicles and robotics, Real time object detection \cite{park2020real}  \\ \hline

% \multicolumn{2}{|c|}{Reference} &
%   & 
%   &
%   &\\ \hline
\end{tabular}%
%}
% \end{table}






% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \begin{table}[]
% \centering
% %\resizebox{\textwidth}{!}{%
% \begin{tabular}{|p{5em}p{5em}|p{10em}|p{12em}|p{10em}|p{10em}|}
% \hline
% \hline
% \multicolumn{2}{|c|}{} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Embedded} \\ \textbf{Edge Devices}\end{tabular}} &
% %\multicolumn{1}{c|}{Embedded Edge Devices} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Nodes {\slash}} \\ \textbf{Edge Servers {\slash}} \\ \textbf{Edge Computers {\slash}} \\ \textbf{Micro Datacenter}\end{tabular}} &
% %\multicolumn{1}{c|}{Edge Nodes {\slash} Edge Servers {\slash} Edge Computers {\slash} Micro Data Center} &
% \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Edge Routers {\slash}} \\ \textbf{Edge Switches {\slash}} \\ \textbf{Edge Gateways}\end{tabular}} &
% %\multicolumn{1}{c|}{Edge Routers {\slash} Edge Switches {\slash} Edge Gateways} &
% \multicolumn{1}{c|}{\textbf{Edge Accelerators}} \\ \hline
% \multicolumn{2}{|c|}{Processing Power} &
%   Micro-processor, Micro-controller; (Low-power   processors) &
%   Quad-Core, Hvbrid-Core (General purpose processors); Intel Atom, Intel Celeron, Xeon Processor; GPU Supported &
%   4 to 56 core processors (Customizable); 2nd Generation Intel Xeon Scalable processors &
%   CPU, GPU, VPU, TPU, FPGA, NPU (Specialized   AI processors) \\ \hline
% \multicolumn{2}{|c|}{Memory} &
%   Up to 8MB; {\newline} SRAM &
%   Up to 256GB; {\newline} DDR4 RDIMM{\slash}LR-DIMM &
%   Up to 64GB;  &
%   Up to 4GB; {\newline} GDDR6, SDRAM, LPDDR4 \\ \hline
% \multicolumn{2}{|c|}{Storage} &
%   Up to 16MB &
%   8GB to 6TB; {\newline} NVMe, SSD, MicroSD, eMMC &
%   Up to 2TB; {\newline} NVMe, SSD, SATA &
%   Up to 16GB; {\newline} eMMC, MicroSD\\ \hline
% \multicolumn{2}{|c|}{Network} &
%   Bluetooth, Wi-Fi &
%   Ethernet, Wi-Fi, Cellular &
%   Ethernet, Wi-Fi, Cellular &
%   Ethernet \\ \hline
% \multicolumn{2}{|c|}{AI Optimization} &
%   Not Supported &
%   Not Supported &
%   Not Supported &
%   Optimized for AI inference \\ \hline
% \multicolumn{2}{|c|}{Power Consumption} &
%   Low power consumption &
%   Moderate power consumption &
%   Moderate power consumption &
%   Moderate to high power consumption \\ \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Durability}} &
%   {\begin{tabular}[c]{@{}c@{}}{Shock \&} \\ {Vibration}\end{tabular}} &
%   % Shock\&Vibration &
%   Some Application Supports &
%   Some Application Supports &
%   Some Application Supports &
%   Not Supported \\ \cline{2-6} 
% \multicolumn{1}{|c|}{} &
%   Temperature &
%   -40C to 85C &
%   -40C to 85C &
%   -20C to 60C &
%   -40C to 85C  \\ \cline{2-6} 
% \multicolumn{1}{|c|}{} &
%   Waterproof &
%   Some Application Supports &
%   Some Application Supports &
%   Some Application Supports &
%   No \\ \hline
% \multicolumn{2}{|c|}{Price} &
%   \$ &
%   \$\$ to \$\$\$ &
%   \$\$ to \$\$\$ &
%   \$\$\$ \\ \hline
% \multicolumn{2}{|c|}{Typical Application} &
%   Sensor devices, wearables, IoT devices, smart appliances\cite{9904804}\cite{8951147} &  
%   Kiosk machines, Building automation, Environmental monitoring, Industrial robotics, Railway signaling systems, Industrial data centers, Smart cities infrastructure\cite{JIANG2020556} &
%   Industrial control systems, Industrial gateways, Smart manufacturing systems &
%   Video surveillance and analytics, Autonomous vehicles and robotics \\ \hline
% \multicolumn{2}{|c|}{Example of Devices} &
%   Arduino &
%   Raspberry Pi, Industrial edge servers, NVIDIA Jetson,Dell Edge Gateway &
%   Cisco IoT routers, Juniper Networks &
%   % NVIDIA Tesla T4, 
%   Google Coral TPU \\ \hline
% \multicolumn{2}{|c|}{I/O} &
%   USB, Ethernet &
%   PCIe, OCP, LOM, USB, iDRAC network port, Display ports &
%   Display ports, USB, uSIM slots, COM, Digital I/O &
%   PCIe, USB, HDMI, uSDHC, GPIO \\ \hline
% % \multicolumn{2}{|c|}{Reference} &
% %   & 
% %   &
% %   &\\ \hline
% \end{tabular}%
% %}
% % \end{table}

==> Contents/tables/testing_results.tex <==
\begin{tabular}{llllll}
\hline\hline
\textbf{Model} & \textbf{Parameters}  & \textbf{Test Acc} & \textbf{Inference Time} & \textbf{Mem Usage} & \textbf{Power Cons} \\
\hline
Xception-Lite & 11.2M & \textbf{73.45\%} & 35s & 1493.1 MB & XXXX \\
MobileNetV2 & 2.2M & 50.05\% & \textbf{22s} & 1745.2 MB & XXXX \\
EfficientNetV2B0 & 5.9M & 54.30\% & 28s & 1451.8 MB & XXXX \\
MobileViT-XXS & \textbf{1.3M} & 50.00\% & 48s & \textbf{1135.7 MB} & XXXX \\
% Xception & 20M & XXXX & 1120s & XXXXX \\
\hline
\end{tabular}


==> Contents/tables/training_results.tex <==
\begin{tabular}{ccccccccc}
\hline\hline
\textbf{Model} & \textbf{Configurations} &\textbf{Parameters}  & \textbf{Train Acc} &\textbf{Test Acc} & \textbf{Avg Time/epoch} & \textbf{Avg Mem Used} & \textbf{Avg GPU Used} & \textbf{Avg Pow Cons}\\
\hline
\textcolor{blue}{Proposed Model} & \textcolor{blue}{no pre-training} & \textcolor{blue}{11.2M} & \textcolor{red}{\textbf{97.93\%}} & \textcolor{red}{\textbf{73.45\%}} & \textcolor{blue}{564.94s} & \textcolor{blue}{0.9074 GB} & \textcolor{blue}{92.84\%} & \textcolor{blue}{18.07W}\\\hline
EfficientNetV2B0 & no pre-training & 5.9M & 84.39\% & 54.30\% & 357.94s & 0.9339 GB & \textcolor{red}{\textbf{85.12\%}} & 16.42W\\
MobileNetV2 & no pre-training & 2.2M & 90.35\% & 50.05\% & \textcolor{red}{\textbf{270.09s}} & \textcolor{red}{\textbf{0.8838 GB}} & 87.14\% & \textcolor{red}{\textbf{15.19W}}\\
MobileViT-XXS & no pre-training & 1.3M & 65.89\% & 67.25\% & 693.81s & 0.9303 GB & 89.77\% & 15.90W\\
% MobileViT-XXS & no pre-training & 1.3M & 95.06\% & \textcolor{red}{\textbf{75.40\%}} & 693.81s & 0.9303 GB & 89.77\% & 15.90W\\
% Xception & 20M & XXXX & 1120s & XXXXX \\
\hline
\end{tabular}


% \begin{tabular}{ccccccccc}
% \hline\hline
% \textbf{Model} & \textbf{Configurations} &\textbf{Parameters}  & \textbf{Train Acc} &\textbf{Test Acc} & \textbf{Avg Time/epoch} & \textbf{Avg Mem Used} & \textbf{Avg GPU Used} & \textbf{Avg Pow Cons}\\
% \hline
% \textcolor{blue}{Xception-Lite} & \textcolor{blue}{no pre-training} & \textcolor{blue}{11.2M} & \textcolor{red}{\textbf{97.93\%}} & \textcolor{red}{\textbf{73.45\%}} & \textcolor{blue}{564.94s} & \textcolor{blue}{0.9074 GB} & \textcolor{blue}{92.84\%} & \textcolor{blue}{18.07W}\\\hline
% EfficientNetV2B0 & no pre-training & 5.9M & 84.39\% & 54.30\% & 357.94s & 0.9339 GB & \textcolor{red}{\textbf{85.12\%}} & 16.42W\\
% MobileNetV2 & no pre-training & 2.2M & 90.35\% & 50.05\% & \textcolor{red}{\textbf{270.09s}} & \textcolor{red}{\textbf{0.8838 GB}} & 87.14\% & \textcolor{red}{\textbf{15.19W}}\\
% MobileViT-XXS & no pre-training & 1.3M & 65.89\% & 67.25\% & 693.81s & 0.9303 GB & 89.77\% & 15.90W\\
% % MobileViT-XXS & no pre-training & 1.3M & 95.06\% & \textcolor{red}{\textbf{75.40\%}} & 693.81s & 0.9303 GB & 89.77\% & 15.90W\\
% % Xception & 20M & XXXX & 1120s & XXXXX \\
% \hline
% \end{tabular}

